TTB: Test-time Baking for Efficient Rendering of Decoder-only View Synthesis Models

Decoder-only Large View Synthesis Models (LVSMs) with KV-cache have recently achieved state-of-the-art quality by regressing novel views from neural networks without reconstructing 3D geometry, while Test-Time Training (TTT) layers save computation but sacrifice quality. We propose Test-Time Baking (TTB), a strategy that learns to bake global scene information from cross-view attention into a lightweight MLP, enabling fast and high-fidelity novel-view decoding. The first key is to repurpose the fast-weight MLP of TTT to learn the cross-view attention mapping explicitly from its input-output pairs, rather than replacing attention entirely, achieving the same rendering efficiency as TTT while delivering substantially higher quality. The second key addresses a modality misalignment between context prefilling and novel-view rendering: we disentangle context tokens into camera-only context rendering tokens to serve as TTB input, and context ground-truth tokens with image content to serve as the TTB mapping target, ensuring the baked MLPs are relieved of the modality generalization challenge between context and novel-view processing. Our method achieves up to **23x** rendering speedup with quality on par with the state-of-the-art across several benchmarks. Project page: https://test-time-baking.github.io

==> tab/ablation_feedback_residual.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\caption{\textbf{TTB layer design ablation on DL3DV.} \emph{Residual} denotes learning the residual $\text{CrossAttn}(X^{(\text{ctx-gt})})-X^{(\text{ctx-rend})}$ as the inner-loop target instead of the absolute cross-view attention output; \emph{Feedback} denotes additionally applying the baked MLP to update the context ground-truth tokens for downstream layers (Fig.~\ref{fig:pipeline}).}
\label{tab:ablation_feedback_residual}
\begin{tabular}{ccccc}
\toprule
Feedback & Residual & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\midrule
\xmark & \xmark & 24.32 & 0.748 & 0.243 \\
\xmark & \cmark & \cellcolor{yellow!25}24.75 & \cellcolor{orange!25}0.764 & \cellcolor{orange!25}0.233 \\
\cmark & \xmark & \cellcolor{orange!25}24.76 & \cellcolor{orange!25}0.764 & \cellcolor{yellow!25}0.231 \\
\cmark & \cmark & \cellcolor{red!25}24.84 & \cellcolor{red!25}0.768 & \cellcolor{red!25}0.230 \\
\bottomrule
\end{tabular}
\end{table}

==> tab/ablation_innerloop.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\caption{\textbf{Inner-loop optimization ablation on DL3DV.}}
\label{tab:ablation_innerloop}
\begin{tabular}{lccccc}
\toprule
Framework & $T$ & Loss & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\midrule
TTT~\cite{lact} & 1 & dot-prod & 23.12 & 0.704 & 0.286 \\
TTT~\cite{lact} & 3 & MSE      & 23.39 & 0.715 & 0.278 \\
\midrule
TTB{-}{-}             & 1 & dot-prod & 23.78 & 0.728 & 0.264 \\
TTB{-}{-}             & 1 & MSE      & 23.85 & 0.731 & 0.261 \\
TTB{-}{-}             & 3 & dot-prod & 23.96 & 0.737 & 0.258 \\
TTB{-}{-}             & 2 & MSE      & \cellcolor{yellow!25}24.16 & \cellcolor{yellow!25}0.744 & \cellcolor{yellow!25}0.251 \\
TTB{-}{-}             & 3 & MSE      & \cellcolor{orange!25}24.22 & \cellcolor{orange!25}0.747 & \cellcolor{orange!25}0.248 \\
TTB{-}{-}             & 5 & MSE      & \cellcolor{red!25}24.29 & \cellcolor{red!25}0.751 & \cellcolor{red!25}0.246 \\
\bottomrule
\end{tabular}
\end{table}

==> tab/ablation_pretrain.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\caption{\textbf{Pretraining ablation across frameworks on DL3DV.}}
\label{tab:ablation_pretrain}
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c}{w/o pretrain} & \multicolumn{3}{c}{w/ pretrain} & \multirow{2}{*}{$\Delta$ PSNR} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & \\
\midrule
TTT~\cite{lact}  & 22.84 & 0.688 & 0.307 & 23.12 & 0.704 & 0.286 & $+0.28$ \\
TTB{-}{-}            & 23.51 & 0.720 & 0.274 & 24.22 & 0.747 & 0.248 & $+0.71$ \\
TTB              & \textbf{23.82} & \textbf{0.731} & \textbf{0.264} & \textbf{24.84} & \textbf{0.768} & \textbf{0.230} & $\mathbf{+1.02}$ \\
\bottomrule
\end{tabular}
\end{table}

==> tab/memory.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{8pt}
\caption{\textbf{Per-scene memory at 960p on a single A100.} Stored size is the scene state held during rendering; peaks are measured during reconstruction and rendering. TTB-duplicate uses $B{=}16$ views per copy, i.e.\ $K{=}V/16$ copies.}
\label{tab:memory}
\begin{tabular}{l l ccc}
\toprule
& Method & $V{=}16$ & $V{=}32$ & $V{=}64$ \\
\midrule
\multirow{4}{*}{Stored size (MB)$\downarrow$}
& DVSM (KV-cache) & 6885 & 13770 & 27540 \\
& TTB{-}{-}       & 324  & 324   & 324 \\
& TTB             & 324  & 324   & 324 \\
& TTB-duplicate   & 324  & 648   & 1296 \\
\midrule
\multirow{4}{*}{Peak recon.\ memory (GB)$\downarrow$}
& DVSM            & 11.4 & 21.7 & 42.5 \\
& TTB{-}{-}       & 10.6 & 19.5 & 37.2 \\
& TTB             & 11.9 & 21.9 & 41.9 \\
& TTB-duplicate   & 11.9 & 22.8 & 48.0 \\
\midrule
\multirow{4}{*}{Peak render.\ memory (GB)$\downarrow$}
& DVSM            & 8.0 & 14.8 & 28.4 \\
& TTB{-}{-}       & 1.9 & 2.0  & 2.2 \\
& TTB             & 2.0 & 2.1  & 2.3 \\
& TTB-duplicate   & 2.0 & 2.4  & 3.3 \\
\bottomrule
\end{tabular}
\end{table}


==> tab/supp_dl3dv_more_split.tex <==
\begin{table}[tb]
\begin{minipage}[t]{.49\linewidth}
  \centering
  \caption{{\bf Additional splits with 256$\times$256 center crop.}}
  \label{tab:dl3dv_difficult_split}
  \centering
  \begin{adjustbox}{max width=\linewidth}
  \begin{tabular}{@{}lrc ccc@{}}
  \toprule
    Method & Venue && PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
  \midrule
    \multicolumn{5}{@{}l}{\bf \underline{DL3DV: \cite{depthsplat}'s split + 4 views}} \\
    DepthSplat~\cite{depthsplat} & CVPR'25
    && 22.30 & 0.765 & 0.189 \\
    LargerNVS~\cite{largernvs} & CVPR'26
    && 27.56 & 0.869 & 0.095 \\
    DVSM~\cite{dvsm} & {\footnotesize anonymized}
    && 26.95 & 0.850 & 0.120 \\
    Ours{-}{-} & 
    && 24.83 & 0.796 & 0.156 \\
    Ours &
    && 26.34 & 0.835 & 0.133 \\
  \midrule
    \multicolumn{5}{@{}l}{\bf \underline{DL3DV: \cite{depthsplat}'s split + 6 views}} \\
    DepthSplat~\cite{depthsplat} & CVPR'25
    && 23.47 & 0.812 & 0.154 \\
    LargerNVS~\cite{largernvs} & CVPR'26
    && 29.45 & 0.904 & 0.068 \\
    DVSM~\cite{dvsm} & {\footnotesize anonymized}
    && 29.40 & 0.902 & 0.082 \\
    Ours{-}{-} & 
    && 28.17 & 0.881 & 0.098 \\
    Ours &
    && 29.12 & 0.899 & 0.087 \\
  \midrule
    \multicolumn{5}{@{}l}{\bf \underline{DL3DV: \cite{rayzer}'s even split + 16 views}} \\
    GSLRM~\cite{gslrm} & ECCV'25
    && 23.49 & 0.712 & 0.252  \\
    LVSM~\cite{lvsm} & ICLR'25
    && 23.69 & 0.723 & 0.242 \\
    Rayzer~\cite{rayzer} & ICCV'25
    && 24.36 & 0.757 & 0.209 \\
    DVSM~\cite{dvsm} & {\footnotesize anonymized}
    && 30.27 & 0.910 & 0.078 \\
    Ours{-}{-} & 
    && 29.45 & 0.898 & 0.090 \\
    Ours &
    && 30.20 & 0.911 & 0.081 \\
  \midrule
    \multicolumn{5}{@{}l}{\bf \underline{DL3DV: \cite{rayzer}'s random split + 16 views}} \\
    GSLRM~\cite{gslrm} & ECCV'25
    && 23.02 & 0.705 & 0.266  \\
    LVSM~\cite{lvsm} & ICLR'25
    && 23.10 & 0.703 & 0.257 \\
    Rayzer~\cite{rayzer} & ICCV'25
    && 23.72 & 0.733 & 0.222 \\
    DVSM~\cite{dvsm} & {\footnotesize anonymized}
    && 30.16 & 0.912 & 0.076 \\
    Ours{-}{-} & 
    && 29.37 & 0.900 & 0.088 \\
    Ours &
    && 30.11 & 0.912 & 0.080 \\
  \bottomrule
  \end{tabular}
  \end{adjustbox}
\end{minipage}
\begin{minipage}[t]{.49\linewidth}
  \centering
  \caption{{\bf Additional splits with 512$\times$512 center crop.}}
  \label{tab:dl3dv_difficult_split}
  \centering
  \begin{adjustbox}{max width=\linewidth}
  \begin{tabular}{@{}lrc ccc@{}}
  \toprule
    Method & Venue && PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
  \midrule
    \multicolumn{5}{@{}l}{\bf \underline{DL3DV: \cite{depthsplat}'s split + 4 views}} \\
    LargerNVS~\cite{largernvs} & CVPR'26
    && 24.94 & 0.780 & 0.188 \\
    DVSM~\cite{dvsm} & {\footnotesize anonymized}
    && 26.22 & 0.825 & 0.168\\
    Ours{-}{-} & 
    && 24.33 & 0.776 & 0.211 \\
    Ours &
    && 24.75 & 0.785 & 0.207 \\
  \midrule
    \multicolumn{5}{@{}l}{\bf \underline{DL3DV: \cite{depthsplat}'s split + 6 views}} \\
    LargerNVS~\cite{largernvs} & CVPR'26
    && 26.14 & 0.808 & 0.159 \\
    DVSM~\cite{dvsm} & {\footnotesize anonymized}
    && 28.75 & 0.880 & 0.120 \\
    Ours{-}{-} & 
    && 27.57 & 0.856 & 0.141 \\
    Ours &
    && 28.73 & 0.881 & 0.121 \\
  \midrule
    \multicolumn{5}{@{}l}{\bf \underline{MipNerf360: \cite{reconfusion}'s split + 3 views}} \\
    LargerNVS~\cite{largernvs} & CVPR'26
    && 18.08 & 0.434 & 0.497 \\
    DVSM~\cite{dvsm} & {\footnotesize anonymized}
    && 16.11 & 0.365 & 0.636 \\
    Ours{-}{-} & 
    && 15.47 & 0.353 & 0.664 \\
    Ours &
    && 15.78 & 0.363 & 0.653 \\
  \midrule
    \multicolumn{5}{@{}l}{\bf \underline{MipNerf360: \cite{reconfusion}'s split + 6 views}} \\
    LargerNVS~\cite{largernvs} & CVPR'26
    && 19.39 & 0.469 & 0.436 \\
    DVSM~\cite{dvsm} & {\footnotesize anonymized}
    && 17.73 & 0.413 & 0.534 \\
    Ours{-}{-} & 
    && 18.00 & 0.424 & 0.516 \\
    Ours &
    && 18.24 & 0.435 & 0.500 \\
  \midrule
    \multicolumn{5}{@{}l}{\bf \underline{MipNerf360: \cite{reconfusion}'s split + 9 views}} \\
    LargerNVS~\cite{largernvs} & CVPR'26
    && 20.39 & 0.493 & 0.402 \\
    DVSM~\cite{dvsm} & {\footnotesize anonymized}
    && 19.02 & 0.459 & 0.470 \\
    Ours{-}{-} & 
    && 19.47 & 0.478 & 0.443 \\
    Ours &
    && 19.95 & 0.501 & 0.414 \\
  \bottomrule
  \end{tabular}
  \end{adjustbox}
\end{minipage}
\end{table}



==> tab/supp_re10k_more_split.tex <==
\begin{table}[tb]
  \centering
  \caption{{\bf Re10k additional split.}}
  \label{tab:re10k_difficult_split}
  \centering
  \begin{adjustbox}{max width=\linewidth}
  \begin{tabular}{@{}lrc ccc@{}}
  \toprule
    Method & Venue && PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
  \midrule
    \multicolumn{5}{@{}l}{\bf \underline{\cite{noposplat}'s split + 2 views + 256$\times$256}} \\
    pixelNeRF~\cite{pixelnerf} & CVPR'21
    && 19.82 & 0.626 & 0.485 \\
    AttnRend~\cite{attnrend} & CVPR'23
    && 22.66 & 0.762 & 0.269 \\
    PixelSplat~\cite{pixelsplat} & CVPR'24
    && 23.85 & 0.806 & 0.185 \\
    MVSplat~\cite{mvsplat} & ECCV'24
    && 23.98 & 0.811 & 0.176 \\
    DVSM & {\footnotesize anonymized}
    && 29.27 & 0.896 & 0.109 \\
    Ours \\
  \midrule
    \multicolumn{5}{@{}l}{\bf \underline{\cite{rayzer}'s even split + 5 views + 256$\times$256}} \\
    GSLRM~\cite{gslrm} & ECCV'25
    && 24.25 & 0.770 & 0.227 \\
    LVSM~\cite{lvsm} & ICLR'25
    && 27.00 & 0.851 & 0.157 \\
    Rayzer~\cite{rayzer} & ICCV'25
    && 27.48 & 0.861 & 0.146 \\
    Ours{-}{-} \\
    Ours \\
  \midrule
    \multicolumn{5}{@{}l}{\bf \underline{\cite{rayzer}'s random split + 5 views + 256$\times$256}} \\
    GSLRM~\cite{gslrm} & ECCV'25
    && 23.21 & 0.748 & 0.251 \\
    LVSM~\cite{lvsm} & ICLR'25
    && 25.88 & 0.828 & 0.175 \\
    Rayzer~\cite{rayzer} & ICCV'25
    && 26.32 & 0.835 & 0.164 \\
    Ours{-}{-} \\
    Ours \\
  \bottomrule
  \end{tabular}
  \end{adjustbox}
\end{table}



==> tab/tmp_dl3dv_internal_only.tex <==
% \begin{table}[tb]
%   \centering
%   \caption{\bf Many input views on DL3DV.}
%   \begin{tabular}{@{}l@{}r@{}c cc c ccc@{}}
%     \toprule
%     Method & Venue &&
%     PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ &&
%     Time$\downarrow$ & FPS$\uparrow$ \\
%     \midrule
%     \multicolumn{8}{@{}l}{\bf \underline{16 input views}}\vspace{.3em} \\
%     3DGS~\cite{3dgs} & ToG'23 &&
%     21.20 & 0.708 & 0.264 &&
%     >600s & >50 \\
%     LVSM~\cite{lvsm}$^\dagger$ & ICLR'25 &&
%     21.64 & 0.666 & 0.365 &&
%     4s & 19.9 \\
%     LongLRM~\cite{longlrm} & ICCV'25 &&
%     22.66 & 0.740 & 0.292 &&
%     0.4s & >50 \\
%     LongLRM++~\cite{longlrmpp} & arxiv'25 &&
%     24.40 & 0.795 & 0.231 &&
%     1.6s & 14\\
%     tttLRM~\cite{tttlrm} & CVPR'26 &&
%     23.60 & 0.784 & 0.255 &&
%     3.6s & -\\
%     LaCT~\cite{lact} & ICLR'26 &&
%     24.70 & 0.793 & 0.224 &&
%     2.2s & 10\\
%     % \multicolumn{2}{@{}l}{DVSM \tiny{ ps16+dino}}
%     % &&
%     % 25.46 & 0.808 & 0.199 &&
%     % 0.6s & 40 \\
%     DVSM &  &&
%     25.88 & 0.823 & 0.188 &&
%     4.4s & 4 \\
%     DVSM+TTB{-}{-} & &&
%     & & &&
%      & 20 \\
%     DVSM+TTB & &&
%     & & &&
%      & 20 \\
%     \midrule
%     \multicolumn{7}{@{}l}{\bf \underline{32 input views}}\vspace{.3em} \\
%     3DGS~\cite{3dgs} & ToG'23 &&
%     23.60 & 0.779 & 0.213 &&
%     >600s & >50 \\
%     LVSM~\cite{lvsm}$^\dagger$ & ICLR'25 &&
%     21.73 & 0.664 & 0.365 &&
%     15s & 20 \\
%     LongLRM~\cite{longlrm} & ICCV'25 &&
%     24.10 & 0.783 & 0.254 &&
%     1s & >50 \\
%     LongLRM++~\cite{longlrmpp} & arxiv'25 &&
%     26.43 & 0.846 & 0.180 &&
%     4.7s & 14\\
%     tttLRM~\cite{tttlrm} & CVPR'26 &&
%     25.07 & 0.822 & 0.215 &&
%     7.2s & -\\
%     LaCT~\cite{lact} & ICLR'26 &&
%     26.90 & 0.837 & 0.185 &&
%     4.3s & 10\\
%     % \multicolumn{2}{@{}l}{DVSM \tiny{ ps16+dino}}
%     % &&
%     % 27.29 & 0.852 & 0.159 &&
%     % 1.8s & 25\\
%     DVSM &  &&
%     27.96 & 0.869 & 0.145 &&
%     15s & 2\\
%     DVSM+TTB{-}{-} & &&
%     & & &&
%      & 20 \\
%     DVSM+TTB & &&
%     & & &&
%      & 20 \\
%     \midrule
%     \multicolumn{7}{@{}l}{\bf \underline{64 input views}}\vspace{.3em} \\
%     3DGS~\cite{3dgs} & ToG'23 &&
%     26.43 & 0.854 & 0.167 &&
%     >600s & >50\\
%     LVSM~\cite{lvsm}$^\dagger$ & ICLR'25 &&
%     21.46 & 0.651 & 0.377 &&
%     60s & 19 \\
%     LongLRM~\cite{longlrm} & ICCV'25 &&
%     24.77 & 0.804 & 0.239 &&
%     3s & >50\\
%     LongLRM++~\cite{longlrmpp} & arxiv'25 &&
%     27.30 & 0.869 & 0.161 &&
%     16s & 14\\
%     tttLRM~\cite{tttlrm} & CVPR'26 &&
%     25.95 & 0.844 & 0.195 &&
%     15s & -\\
%     LaCT~\cite{lact} & ICLR'26 &&
%     28.30 & 0.857 & 0.169 &&
%     8.7s & 10\\
%     % \multicolumn{2}{@{}l}{DVSM \tiny{ ps16+dino}}
%     % &&
%     % 28.90 & 0.882 & 0.135 &&
%     % 5.2s & 15\\
%     DVSM &  &&
%     29.71 & 0.898 & 0.120 &&
%     60s & 1\\
%     DVSM+TTB{-}{-} & &&
%     & & &&
%      & 20 \\
%     DVSM+TTB & &&
%     & & &&
%      & 20 \\
%   \bottomrule
%   \end{tabular}
% \end{table}

\begin{table}[tb]
  \centering
  \caption{\bf Many input views on DL3DV.}
  \begin{tabular}{@{}l@{}r@{}c cc c ccc@{}}
    \toprule
    Method &  &&
    PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ &&
    Time$\downarrow$ & FPS$\uparrow$ \\
    \midrule
    \multicolumn{8}{@{}l}{\bf \underline{16 input views}}\vspace{.3em} \\
    3DGS~\cite{3dgs} &  &&
    21.20 & 0.708 & 0.264 &&
    >600s & >50 \\
    LVSM~\cite{lvsm}$^\dagger$ &  &&
    21.64 & 0.666 & 0.365 &&
    4s & 19.9 \\
    LongLRM~\cite{longlrm} &  &&
    22.66 & 0.740 & 0.292 &&
    0.4s & >50 \\
    LongLRM++~\cite{longlrmpp} &  &&
    24.40 & 0.795 & 0.231 &&
    1.6s & 14\\
    tttLRM~\cite{tttlrm} &  &&
    23.60 & 0.784 & 0.255 &&
    3.6s & -\\
    LaCT~\cite{lact} &  &&
    24.70 & 0.793 & 0.224 &&
    2.2s & 10\\
    % \multicolumn{2}{@{}l}{DVSM \tiny{ ps16+dino}}
    % &&
    % 25.46 & 0.808 & 0.199 &&
    % 0.6s & 40 \\
    DVSM &  &&
    25.88 & 0.823 & 0.188 &&
    4.4s & 4 \\
    DVSM+TTB{-}{-} & &&
    & & &&
    1.9s & 23 \\
    DVSM+TTB & &&
    & & &&
    5.4s & 23 \\
    \midrule
    \multicolumn{7}{@{}l}{\bf \underline{32 input views}}\vspace{.3em} \\
    3DGS~\cite{3dgs} &  &&
    23.60 & 0.779 & 0.213 &&
    >600s & >50 \\
    LVSM~\cite{lvsm}$^\dagger$ &  &&
    21.73 & 0.664 & 0.365 &&
    15s & 20 \\
    LongLRM~\cite{longlrm} &  &&
    24.10 & 0.783 & 0.254 &&
    1s & >50 \\
    LongLRM++~\cite{longlrmpp} &  &&
    26.43 & 0.846 & 0.180 &&
    4.7s & 14\\
    tttLRM~\cite{tttlrm} &  &&
    25.07 & 0.822 & 0.215 &&
    7.2s & -\\
    LaCT~\cite{lact} &  &&
    26.90 & 0.837 & 0.185 &&
    4.3s & 10\\
    % \multicolumn{2}{@{}l}{DVSM \tiny{ ps16+dino}}
    % &&
    % 27.29 & 0.852 & 0.159 &&
    % 1.8s & 25\\
    DVSM &  &&
    27.96 & 0.869 & 0.145 &&
    15s & 2\\
    DVSM+TTB{-}{-} & &&
    & & &&
    3.7s & 23 \\
    DVSM+TTB & &&
    & & &&
    18s & 23 \\
    \midrule
    \multicolumn{7}{@{}l}{\bf \underline{64 input views}}\vspace{.3em} \\
    3DGS~\cite{3dgs} &  &&
    26.43 & 0.854 & 0.167 &&
    >600s & >50\\
    LVSM~\cite{lvsm}$^\dagger$ &  &&
    21.46 & 0.651 & 0.377 &&
    60s & 19 \\
    LongLRM~\cite{longlrm} &  &&
    24.77 & 0.804 & 0.239 &&
    3s & >50\\
    LongLRM++~\cite{longlrmpp} &  &&
    27.30 & 0.869 & 0.161 &&
    16s & 14\\
    tttLRM~\cite{tttlrm} &  &&
    25.95 & 0.844 & 0.195 &&
    15s & -\\
    LaCT~\cite{lact} &  &&
    28.30 & 0.857 & 0.169 &&
    8.7s & 10\\
    % \multicolumn{2}{@{}l}{DVSM \tiny{ ps16+dino}}
    % &&
    % 28.90 & 0.882 & 0.135 &&
    % 5.2s & 15\\
    DVSM &  &&
    29.71 & 0.898 & 0.120 &&
    60s & 1\\
    DVSM+TTB{-}{-} & &&
    & & &&
    7.5s & 23 \\
    DVSM+TTB & &&
    & & &&
    65s & 23 \\
  \bottomrule
  \end{tabular}
\end{table}




